Structured Knowledge Grounding for Question Answering

Can language models (LM) ground question-answering (QA) tasks in the knowledge base via inherent relational reasoning ability? While previous models that use only LMs have seen some success on many QA tasks, more recent methods include knowledge graphs (KG) to complement LMs with their more logic-driven implicit knowledge. However, effectively extracting information from structured data, like KGs, empowers LMs to remain an open question, and current models rely on graph techniques to extract knowledge. In this paper, we propose to solely leverage the LMs to combine the language and knowledge for knowledge based question-answering with flexibility, breadth of coverage and structured reasoning. Specifically, we devise a knowledge construction method that retrieves the relevant context with a dynamic hop, which expresses more comprehensivenes than traditional GNN-based techniques. And we devise a deep fusion mechanism to further bridge the information exchanging bottleneck between the language and the knowledge. Extensive experiments show that our model consistently demonstrates its state-of-the-art performance over CommensenseQA benchmark, showcasing the possibility to leverage LMs solely to robustly ground QA into the knowledge base.

==> sections/2-related.tex <==
\section{Related Works}
\subsection{Knowledge Grounded Question Answering}
Knowledge grounded question answering is an emerging topic and the current state-of-the-art large language models are still struggling with this task.
~\cite{lin2019kagnet} proposed a textual inference framework to solve commonsense-related questions by leveraging external, structured commonsense knowledge graphs to perform explainable inferences.
Many recent works explore to leverage the knowledge base to enhance the question answering task.

\subsection{Knowledge Graph Fusion for Language Models}
Knowledge can be stored implicitly in huge language models like GPT-$2$ and BERT that have been pre-trained on raw texts, or explicitly in knowledge graphs like FreeBase~\cite{bollacker2008freebase} and ConceptNet~\cite{liu2004conceptnet}. Many QA tasks have already seen remarkable success due to pre-trained LMs. Despite their flexibility and breadth of coverage, LMs are unable to construct an organized reasoning flow across contexts, compromising their empirical performance. KGs, on the other hand, are well-suited to structured reasoning, although graphs can be unreliable and noisy. As a result, combining two knowledge sources appears to be a good avenue to pursue.
Previous work~\citep{das-etal-2017-question, sun-etal-2018-open} demonstrate the success of fusing text and knowledge-base for the QA tasks.
More recent work~\citep{agarwal-etal-2021-knowledge, oguz-etal-2022-unik} explore knowledge-enhanced language model pre-training and achieve significant improvement in question answering tasks.
Inspiring by the ubiquitous success of the Transformer architectures, ~\cite{ying2021transformers} built their Graphormer, and attained excellent results on a broad range of graph representation learning tasks.
Both QA-GNN~\cite{Yasunaga2021QAGNNRW} and GreaseLM~\cite{greaseLM} retrieve a subgraph using entity matching and path finding techniques following by jointly reasoning over both modalities by either adding question context to the subgraph as an additional node or introducing additional interaction tokens and layers into the model architecture.

